Projective differential geometry and asymptotic analysis in General Relativity

In this text, we explore the tools that Projective Differential Geometry can provide for the asymptotic analysis of classical fields on projectively compact manifolds. We emphasise on the case of order 2-compactifications and develop, in this case, a projective exterior differential tractor calculus that is analogous to that existing for conformally compact manifolds.

==> annexe/formes_differentielles_valeurs_vectorielles.tex <==
% !TEX root = ../smf_proj.tex
\chapter{Vector valued differential forms}
\label{annexe:formes_tensorielles}

In the literature on principal connections, we are inevitably confronted with the notion of vector valued differential forms. In this appendix, for completeness, we recall some of the definitions and vocabulary useful for the main text and that one comes across in textbooks on the topic. We will mainly follow~\cite{Bleeker:2005aa}, who adopts a point of view close to that predominant in Physics literature. We will also discuss equivalent ways to think about so-called \enquote{basic} or \enquote{tensorial} forms and forms with values in a vector bundle $V$ over $M$.

\section{Definitions}
\begin{defi}
Let $V$ be a fixed finite dimensional vector space and $P$ a smooth manifold, a $V$-valued differential form is a section of the vector bundle : $$\Lambda^k(P,V)=\Lambda^k(T^*P)\otimes(P\times V).$$
If $(P,\pi,M)$ is a $G$-principal fibre bundle and $(V,\rho)$ is a representation of $G$ we will say that $\alpha\in \Gamma(\Lambda^k(P,V))$ is:
\begin{itemize}
\item \emph{equivariant} if $R_g^*\alpha=\rho(g)^{-1}\alpha$,
\item \emph{horizontal} if for all vector fields on $P$ $(X_1,\dots,X_k)$, at least one of which vertical, then $\alpha(X_1,\dots,X_k)=0.$ 
\end{itemize}
A form that is both horizontal and equivariant is said to be \emph{tensorial}.
\end{defi}

\begin{prop}
Let $(P,\pi,M)$ be a $G$-principal fibre bundle, and $(V,\rho)$ a finite dimensional representation of $G$. A tensorial $V$-valued differential form on $P$ is equivalent to a section of the vector bundle over $M$:
\[\Lambda^k(T^*M)\otimes(P\times_G V).\]
\end{prop}
\begin{proof}
Let us first point out that the base of the bundle $\Lambda^k(T^*M)\otimes(P\times_G V)$ is indeed $M$ and not $P$. The equivalence is quite clear in one direction, if we allow ourselves to choose a connection on $P$. In this case, the projection $\pi$ of $P$ induces a vector space isomorphism: $$\textrm{d}\pi_p : H_p \subset T_p P \rightarrow T_{\pi(p)}M,$$ which enables us to horizontally lift vector fields over $M$ to vector fields over $P$. If $X$ is a vector field over $M$, let us call $\tilde{X}$ its horizontal lift. We will also denote by $\textsf{p}$ the canonical projection mapping $P\times V$ onto $P\times_G V$ (cf.  Appendix~\ref{sec:fibre_associe}). With these notations, if $\alpha$ is a tensorial $k$-form over $P$ then for any vector fields $X_1,\dots, X_k$ over $M$, $x\in M$ and $p\in \pi^{-1}(\{x\})$, the equation~:
\[\alpha_{M,x}(X_1,\dots,X_k)=\textsf{p}(\alpha_p(\tilde{X}_1,\dots,\tilde{X}_k)),\]
is independent of the choice of $p$ and the horizontal lift and thus defines a section of $\Lambda^k(T^*P)\otimes (P\times_G V)$.

The other direction is slightly more subtle. Let $\alpha_M$ be a section of $\Lambda^k(T^*M)\otimes(P\times_G V)$.  Of course, the idea is to consider the pullback of $\alpha$ by the projection $\pi$, $\pi^*\alpha_M$, however,  $\pi^*\alpha_M$ is \emph{a priori} only a section of $ \Lambda^k(T^*P)\otimes\pi^*(P\times_G V)$, where~:
$\pi^*(P\times_G V)$ is the pullback bundle of $P\times_G V$ by $\pi$ defined by~:
\[\begin{aligned}\pi^*(P\times_G V) &= \left\{ (p,v), \in P \times (P\times_G V), \tilde{\bar{\pi}}(v)= \pi(p)\right\},\\&\cong \coprod_{p\in P} \left\{ (p,v),v\in (P\times_G V)_{\pi(p)}\right\}.\end{aligned}\]
In the above, we have borrowed notation from Appendix~\ref{sec:fibre_associe} and have introduced the projection $P\times_G V \rightarrow M$, $\tilde{\bar{\pi}}$. The remainder of the proof is dedicated to showing that the bundle $\pi^*(P\times_G V)$ is in fact trivial. Let $r\in P$ and set~:
\[\tilde{\rho}(r): \begin{array}{lcl} V &\longrightarrow& \tilde{\bar{\pi}}^{-1}(\{\pi(r)\})  \\ v & \longmapsto & \textsf{p}((r,v)).\end{array}\]
As for any $v\in V, g\in G$, $\textsf{p}((rg,v))=\textsf{p}((r,\rho(g)v))$, one has~:
\[\tilde{\rho}(rg)=\tilde{\rho}(r)\rho(g).\]
One can then define a map from  $\pi^*(P\times_G V)$ into $P\times V$ by~:
\begin{equation} \label{eq:parallel_pullback_bundle} (p,v)\mapsto (p,\tilde{\rho}(p)^{-1}v).\end{equation}
We leave the proof of the smoothness of our maps to the reader. Minus this detail, the above shows that $\pi^*(P\times_G V)$ is actually parallelisable, because the vector bundle morphism defined by~\eqref{eq:parallel_pullback_bundle} is a vector space isomorphism on each of the fibres. The explicit form of the map shows that, after untangling the pullback bundle, $\pi^*\alpha_M$ is indeed a tensorial form on $P$.
\end{proof}

\section{A few usual operations}
\subsection{The case of a Lie algebra}
Let $\mathfrak{g}$ be a Lie algebra, with bracket $[\phantom{x},\phantom{y}]$. For $\mathfrak{g}$ valued differential forms, there is a natural generalisation of the wedge product. Let $\alpha$ and $\beta$ be respectively $\mathfrak{g}$ valued $k$-form and $l$-form, one defines~: 
\[[\alpha \wedge \beta](X_1,\dots,X_{k\!+\!l})=\frac{\!\!\displaystyle\sum_{\sigma\in\mathfrak{S}_{k+l}}\!\!\!\!\varepsilon(\sigma)[\alpha(X_{\sigma\!(\!1\!)},\dots,X_{\sigma\!(\!k\!)}),\beta(X_{\sigma\!(\!k\!+\!1\!)},\dots,X_{\sigma(k\!+\!l)})]}{k!l!}.\]
In the special case that $\mathfrak{g}$ is a Lie subalgebra of the usual matrix algebra $\mathfrak{gl}_n(\mathbb{R})$ then in fact~:
\[[\alpha\wedge\beta]=\alpha\wedge\beta - (-1)^{kl}\beta\wedge \alpha,\]
where $\alpha\wedge\beta$ is matrix product where component-wise multiplication is replaced by the usual wedge product.
\subsection{Exterior covariant derivative}
Let $(P,\pi,M)$ be a $G$-principal bundle, $V$ a finite dimensional vector space, $\alpha$ a $V$-valued  $k$-form on $P$, and, $(E_i)$ an arbitrary basis of $V$. Writing $\alpha= \alpha^iE_i$, one sets:
\[\textrm{d}\alpha=\textrm{d}\alpha^i E_i.\]
This definition is, in fact,  independent of the choice of basis and inherits all the usual properties of the exterior derivative on forms. When there is a connection, $\omega$, on $P$ we can define a covariant exterior derivative that sends tensorial forms to tensorial forms. Indeed, call the horizontal component of an arbitrary vector $X$, $X^H$ and set~:
\[\textrm{d}^{\omega}\alpha(X_1,\dots,X_n)=\textrm{d}\alpha(X_1^H,\dots,X_n^H).\]
$\textrm{d}^{\omega}\alpha$ is clearly horizontal and one can check equivariance as follows :
\[R_g^*\textrm{d}\alpha=\textrm{d}R_g^*\alpha=\rho(g^{-1})\textrm{d}\alpha.\]

If $\rho$ is a representation and $\rho_*$ is the induced Lie-algebra homomorphism $\mathfrak{g} \rightarrow \mathfrak{gl}(V)$ then for a $V$-valued tensorial $k$-form $\alpha$, and an arbitrary $\mathfrak{g}$ valued $l$-form, $\beta$ one can define:
\[\beta \dot{\wedge}\alpha(X_1, \dots, X_{k\!+\!l})\!=\!\frac{\displaystyle\sum_{\sigma \in \mathfrak{S}_{k+l}}\!\!\!\varepsilon(\sigma) \rho_*(\beta(X_{\sigma\!(\!1\!)},\dots,X_{\sigma\!(\!l\!)}))\!\cdot\!\alpha(X_{\sigma\!(\!l\!+\!1\!)},\dots,X_{\sigma\!(\!l\!+\!k\!)})}{k!l!}.\]
This leads to a useful formula for the exterior covariant derivative: 
\begin{lemm}
\label{lemme:ext_cov_d}
Let $(P,\pi,M)$ be a $G$-principal bundle, $\omega$ a principal connection on $P$, $V$ a finite dimensional vector space, $\rho: G\rightarrow GL(V)$ a representation and  $\alpha$ a $V$-valued tensorial $k$-form on $P$,  then :
\begin{equation}d^{\omega}\alpha = d\alpha + \omega \dot{\wedge}\alpha. \end{equation}
\end{lemm}



==> annexe/principal.tex <==
%!TEX root = ../smf_proj.tex
\chapter{Principal fibre bundles}\label{sec:fibreprincipal}
\section{Definition}
Principal fibre bundles offer a unified perspective of many of the geometric concepts on manifolds. Spinors, tractors, densities and even usual tensors can all be described in a particularly efficient manner in terms of a fibre bundle. They can also be used to give a more general definition of the notion of connection. Without further a-due, here is the definition.
\begin{defi}\label{def:fibreprincipal}
Let $G$  be a Lie group and $M$ a smooth manifold. A $G$-principal fibre bundle with base $M$, written $(P,\pi,M)$ or $(P,G,\pi,M)$, is a smooth manifold $P$ equipped with a smooth surjective map $\pi: P \rightarrow M$ and a smooth right-action of $G$ on $P$ that satisfies:
\begin{itemize}
\item For any $x\in M$, there is an open neighbourhood $U$ of $x$ and a diffeomorphism $\phi: \pi^{-1}(U)\rightarrow U\times G$ such that:
\[\phi(p\cdot g)=\phi(p)\cdot g,\]
where, on the right-hand side, $\phi(p)\cdot g$ is the canonical right action of $G$ on $U\times G$. Such an open neighbourhood $U$ will be called a \enquote{trivialising neighbourhood} and the couple $(\phi,U)$ \enquote{bundle chart}.
\item If $\pi_U: U \times G\rightarrow U$ denotes the canonical projection, then:
\[\pi_U(\phi(p))=\pi(p).\]
\end{itemize}
When the base manifold is clear from the context, we will simply write $(P,\pi)$ or $(P,G,\pi)$. Finally,
when $x \in M$, the set $\pi^{-1}(\{x\})$ is called the \enquote{fibre above $x$}. 
\end{defi}

Before discussing a fundamental and illuminating example, let us first quote the following properties:
\begin{prop}
In the notation of the definition:
\begin{enumerate}
\item The right-action of $G$ on $P$ preserves the fibres in the sense that for any $p\in P, g \in G$, we have: $\pi(pg)=\pi(p)$.
\item $G$ acts freely on $P$.
\item $\pi^{-1}(\{\pi(p)\})$ is the orbit of $p$ under the action of $G$.
\end{enumerate}
\end{prop} 
\begin{proof}
\begin{enumerate}
\item Let $p\in P$, and choose a bundle chart $(\phi,U)$ near $\pi(p)$, then: 
\[\phi(p)g=\phi(pg),\]
so $pg \in \pi^{-1}(U)$. Moreover: \[\begin{aligned} \pi_U(\phi(p)g)&=\pi_U(\phi(p))=\pi(p),\\ \pi_U(\phi(p)g)&=\pi_U(\phi(pg))=\pi(pg), \end{aligned}\] which proves the first point.
\item Let $p\in P$, $g\in G$ that stabilises $p$ and $(\phi,U)$ a bundle chart. By assumption, $pg=p$ so $\phi(pg)=\phi(p)$, hence: $\phi(pg)=\phi(p)g=\phi(p)$ and $g$ fixes $\phi(p)$ in $U\times G$. Since the canonical right-action of  $G$ on $U\times G$ is free, it follows that $g=e.$
\item Fix $p\in P$, since $\pi(pg)=\pi(p)$, $\{ pg, g\in G\} \subset \pi^{-1}(\{\pi(p)\}).$ For the other inclusion, choose $r\in \pi^{-1}(\{\pi(p)\})$ and $(\phi,U)$ a bundle chart near $\pi(p)=\pi(r)=x$. Write, $\phi(r)=(x,g')$ and $\phi(p)=(x,g), g,g' \in G$, then: $\phi(r)=\phi(p)g^{-1}g'=\phi(pg^{-1}g').$ Thus, since $\phi$ is injective, $r=pg^{-1}g'.$
\end{enumerate}
\end{proof}
The final point of the preceding Proposition implies that each of the fibres of $P$ is diffeomorphic (as a manifold), in a non-canonical way, to the group $G$. Just like in affine space there is no privileged choice of identity and the fibres do not have a canonical group structure. To clarify further this structure, we shall now introduce a model example.
%
\section{The frame bundle of a vector bundle}
\label{fibrereperes}
In this section we will discuss how to naturally associate with any vector bundle $(E,\pi_E,V)$ with base $M$ and $m$-dimensional fibre $V$, a $GL(V)$-principal fibre bundle $L(E)$ over $M$, called the \enquote{frame bundle} of $E$.
A generic fibre $L(E)_x$ over a point $x\in M$ will intuitively be the set of all linear frames of the fibre $E_x=\pi_E^{-1}(\{x\})$. Formally, we set:
\begin{equation} 
L(E)=\left\{ (x,u_x), x\in M, u_x \in GL(V,E_x)\right\}.
\end{equation}
The projection map for the principal bundle, $\pi$, is defined by $\pi(x,u_x)=x$ and we shall make $GL(V)$ act from the right on $L(E)$ according to the equation: \[(x,u_x)g = (x,u_x\circ g), g\in GL(V).\]
%
In order to make $L(E)$ into a smooth fibre bundle, we need to ascribe it a topology and differential structure. To this end, consider a bundle atlas $\mathscr{A}$ of $E$, i.e. a family of (vector) bundle charts $(\psi,U)$ where $\psi: \pi_E^{-1}(U) \rightarrow U\times V$ is a diffeomorphism such that for each $x\in U$ the restriction of $\phi$ to the fibre $E_x$ above $x$ induces a vector-space isomorphism between $E_x$ et $V$, and, where $U$ runs over an open cover of the base $M$.
For each chart $(\psi,U)$, define a family of isomorphisms  $\alpha_x \in GL(V,E_x), x\in U$ by $v\mapsto \phi^{-1}(x,v)$ and set: \begin{equation} \tilde{\psi}: \begin{array}{rcr}\pi^{-1}(U) &\longrightarrow& U\times GL(V) \\ (x,u_x) &\longmapsto& (x,\alpha_x^{-1}\circ u_x) \end{array}. \end{equation}
%
$\tilde{\psi}$ is easily seen to be bijective, and:
\[\mathscr{B}= \left\{ \tilde{\psi}^{-1}(O), (\psi,U) \in \mathscr{A}, O \subset U\times GL(V) \textrm{ open }  \right\},\] is a basis for a topology on $L(E)$ which promotes each $\tilde{\psi}$ to a homeomorphism. About each point $p\in L(E)$ one can shrink $U$ so that is the domain of some coordinate chart $(\phi,U)$ on $M$ and construct a local chart $\bar{\psi} : \psi^{-1}(U) \rightarrow \phi(U) \times GL(V)$ by composing $\tilde{\psi}$ with: 
\[\begin{array}{rcl} \phi \times \textrm{Id}_{GL(V)} : U\times G &\longrightarrow& \phi(U) \times G, \\ (x,g)& \longmapsto&(\phi(x),g). \end{array}\]
This specifies a differential atlas that makes the $\tilde{\psi}$ diffeomorphisms.

It follows from our discussion that on each smooth $n$-dimensional manifold $M$, one can construct a $GL_n(\mathbb{R})$-principal fibre bundle: the linear frame bundle of its tangent bundle $TM$. In the sequel, we will see how one can describe the usual tensor bundles over $TM$ using $GL_n(\mathbb{R})$ and how to construct new vector bundles.

\section{Principal connections}
\label{sec:principal_conn}
We come now to the important topic of connections on a principal fibre bundle. In theoretical physics, fibre bundles are used to write down gauge theories, and the notion of connection we now seek to define enables the definition of a covariant derivative for particle fields. In geometry, connections (on the frame bundle) are used to define geodesics and curvature. There are at least three equivalent definitions of a connection, each with its own conceptual or computational advantages. In order to introduce the first definition, we shall first translate into the language of fibre bundles the more familiar notion of affine connection that is used in classical texts on Differential Geometry. We recall first, for instance from~\cite{Carmo:1992aa}, the following definition:
\begin{defi}
\label{def:connexion_carmo}
An affine connection on the tangent bundle is a map: $\nabla: \Gamma(TM)\times \Gamma(TM) \rightarrow \Gamma(TM)$ such that:
\begin{enumerate}
\item For any $Y\in \Gamma(TM)$, $X\mapsto \nabla_X Y$ is a linear endomorphism of the $C^{\infty}(M)$-module $\Gamma(TM)$ of vector fields over $M$,
\item For each $X,Y\in \Gamma(TM)$ and $f \in C^{\infty}(M)$, $\nabla_X(fY)= X(f)Y + f\nabla_XY$.
\end{enumerate}
\end{defi}
Using Penrose's abstract index notation~\cite{Penrose:1984aa}, a connection is therefore an operator $\nabla_a $ that, for any vector field $X^b$ and smooth function $f$, satisfies:
\[\nabla_a(fX^b)=(\nabla_a f) X^b + f\nabla_a X^b,\]
where $\nabla_a f$ is simply the differential of $f$.
%
\section{Affine connection and local moving frames }
Consider now an open set $U\subset M$ and $(e_1,\dots,e_n)$ an $n$-tuple of smooth vector fields defined on $U$ such that for each $x \in U$, $(e_1(x),\dots, e_n(x))$ is a basis of the tangent space $T_xM$. We will now switch Penrose's abstract index notation. Each vector field $X^a$ on $U$ can be written $X^a=X^{\bm{a}}e^a_{\bm{a}}$, where the $X^{\bm{a}}$ are smooth functions on $U$. Let us calculate $\nabla_b X^a$:
\begin{equation}
\label{eq:connexion_generale}
\begin{aligned}
\nabla_b X^a= \nabla_b(X^{\bm{a}}e^a_{\bm{a}})&=(\nabla_b X^{\bm{a}})e^a_{\bm{a}} + X^{\bm{a}} \nabla_be^{a}_{\bm{a}},
\\&=(\nabla_b X^{\bm{a}})e^a_{\bm{a}} +  e_{c}^{\bm{a}}\nabla_be^{c}_{\bm{d}}X^{\bm{d}}e^a_{\bm{a}}.
\end{aligned}
\end{equation}
%Dans~\eqref{eq:connexion_generale} nous avons utilisé la notation $(e^{\bm{c}}_c)$ pour désigner la base duale de $(e^c_{\bm{c}})$. 
It transpires from the final equation that the local action of the affine connection can be described in terms of the matrix of differential forms ${\omega^{\bm{a}}_{\,\,\bm{d}}}_b= e_{c}^{\bm{a}}\nabla_be^{c}_{\bm{d}}$. This can equivalently be seen as a differential form with values in $M_n(\mathbb{R})$\footnote{i.e. a section of the vector bundle $\Lambda^1(T^*U)\otimes(M\times M_n(\mathbb{R}))$, see also Appendix~\ref{annexe:formes_tensorielles}.} that we will call a: \enquote{local connection form}. 

To picture this, one can imagine the data contained in the vector fields $(e^a_{\bm{a}})$ as attaching a local frame of the tangent space to each point $x\in U$ that \enquote{moves} smoothly as $x$ varies.
The \enquote{infinitesimal} change in the frame as it moves from $x$ to a point $x+\delta x$, to first order in $\delta x$, is described by an element of $M_n(\mathbb{R})=\mathfrak{gl}_n(\mathbb{R})$, the Lie algebra of $GL_n(\mathbb{R})$, which corresponds to: $(\omega^{\bm{a}}_{\,\,\bm{d}})$.  % Le premier terme dans~\eqref{eq:connexion_generale} décrit donc la variation infinitésimale des coordonnées du champ $X^a$ exprimé dans ce repère mobile et le deuxième terme décrit celle des vecteurs du repère. En termes du vecteur coordonnées $(X^{\bm{a}})$ du champ $X^a$ dans ce repère mobile, on obtient celui de $\nabla_b X^a$ en dérivant composante par composante, puis en ajoutant le résultat du produit matriciel ${\omega^{\bm{a}}_{\,\,\bm{d}}}_b X^{\bm{d}}$.

A natural question arising now is: given two non-disjoint open sets $U$ and $V$ and two moving frames  $(e_i)$ and $(\tilde{e}_i)$ on $U$ and $V$ respectively, what relation exists between the two corresponding local connection forms $\omega=(\omega^i_{\,\,j})$ and $\tilde{\omega}=(\tilde{\omega}^i_{\,\, j})$ on $U\cap V$?
To answer this, let us define for each $x\in U\cap V$, $P(x)=(P^i_j(x))$ the change of basis matrix from  $(e_i(x))$ to $(\tilde{e}_i(x))$, and denote by $Q^i_j(x)$ its inverse. Let $X$ be a fixed vector field defined on $U\cap V$, one has:
%
\begin{equation} \label{eq:chg_form_connexion_ex} \begin{aligned} \tilde{\omega}^{i}_{\,\,j}(X)=\tilde{e}^i(\nabla_X \tilde{e}_j)&=Q^i_me^m\nabla_X(P^k_je_k),\\&=Q^i_mX(P^k_j)\underbrace{e^m(e_k)}_{\delta^m_k}+Q^i_m\omega^m_{\,\, k}(X)P^k_j,\\&=Q^i_mX(P^m_j)+Q^i_m\omega^m_{\,\, k}(X)P^k_j.\end{aligned} \end{equation}
Denoting by $dP(x)$ the matrix whose coefficients are the differentials of those of $P(x)$
we can rewrite~\eqref{eq:chg_form_connexion_ex}:
%
\begin{equation}\label{eq:transition_form_ex}\tilde{\omega}(X)=P^{-1}dP(X)+P^{-1}\omega(X)P. \end{equation}
This short analysis shows that an affine connection in the sense of Definition~\ref{def:connexion_carmo} can be encoded in a family of matrix valued forms, satisfying the compatibility condition~\eqref{eq:transition_form_ex}, defined on a bundle atlas of $M$. It is easily seen that if $(e_i)$ is a coordinate basis $\frac{\partial}{\partial x_i}$ associated to some local chart, then $(\omega^i_j)$ encodes the familiar Christoffel symbols.

Furthermore, the two terms on the right-hand side of~\eqref{eq:transition_form_ex} have a natural interpretation in terms of the multiplication in the Lie group $GL_n(\mathbb{R})$.
If $g \in GL_n(\mathbb{R})$ then define the maps:
\begin{itemize} 
\item $L_g: A \in GL_n(\mathbb{R}) \mapsto g A$ 
\item $Ad_g$: $A\mapsto gAg^{-1}$,
\item $\mathfrak{ad}_g \in L(\mathfrak{gl}(\mathbb{R}))$ the differential at $Id$ of $Ad_g$.
\end{itemize}
The map $L_g$ gives rise to a canonical $\mathfrak{gl}_n(\mathbb{R})$-valued differential form\footnote{which also gives a global trivialisation of the tangent bundle of $GL_n(\mathbb{R})$} on $GL_n(\mathbb{R})$ defined by:
\[ \theta(X)(g)=d{L_{g^{-1}}}_g(X_g),\]
for any vector field $X\in \Gamma(TGL_n(\mathbb{R}))$. This form is known as the \enquote{Maurer-Cartan form}. We note at this point that none of these objects are specific to $GL_n(\mathbb{R})$ and can be defined \emph{mutatis mutandis} on any Lie group $G$. Nevertheless, for matrix Lie groups, for which the tangent spaces can be identified with vector subspaces of $M_n(\mathbb{R})$, these maps are easily determined. In particular,~\eqref{eq:transition_form_ex} can in fact be written for any $x\in U\cap V$:
\begin{equation} \tilde{\omega}_x= (P^*\theta)_x + \mathfrak{ad}_{P^{-1}(x)}(\omega_x).\end{equation}
In the above formula, $P^*$ is the pullback of the Maurer-Cartan form $\theta$ by the map $x \mapsto P(x)$, i.e. $(P^*\theta)_x(X_x)=\theta_{P(x)}(dP_x\cdot X_x)$, for each $x\in U\cap V, X_x\in T_xM$. We justify the first term: let $X_x \in T_xM$ and $\gamma$ be a smooth curve such that $\gamma(0)=x, \dot{\gamma}(0)=X_x$ then:
\[dP_x(X_x)=\left.\frac{\textrm{d}}{\textrm{d}t}P(\gamma(t))\right|_{t=0}.\]
Furthermore: $t\mapsto P(\gamma(t))$ is a curve $\tilde{\gamma}$ in $GL_n(\mathbb{R})$ that satisfies $\tilde{\gamma}(0)=P(x)$ and $\dot{\tilde{\gamma}}(0)=\left.\frac{\textrm{d}}{\textrm{d}t}P(\gamma(t))\right|_{t=0}$, therefore:
\[\begin{aligned} (P^*\theta)_x(X_x)&=d{L_{P(x)^{-1}}}_{P(x)}(dP_x(X_x))= \frac{\textrm{d}}{\textrm{d}t}\left(P(x)^{-1}P(\gamma(t))\right)\\&=P(x)^{-1}dP_x(X_x).\end{aligned}\]
Up to now, we have yet to discuss what any of this has to do with $L(TM)$. We first need to introduce a little extra material.

\section{Local sections of a principal fibre bundle, transition functions}
\begin{defi}
Let $(P,G,\pi,M)$ be a principal fibre bundle, and $U$ an open subset of $M$. A local section of $P$ on $U$ is a smooth map $\sigma_U: U \rightarrow P$ such that for each $x\in U$, $\pi(\sigma_U(x))=x$.
\end{defi}

\begin{prop}
\label{prop:section_locale}
Retaining the notation introduced in the previous definition, any local section on $U$ determines a local bundle chart $(\psi,U)$ and, conversely, every local bundle chart $(\psi,U)$ determines a local section.
\end{prop}
\begin{proof}
If $\sigma_U$ is a local section, define $\psi: \pi^{-1}(U) \rightarrow U\times G$ by: $$\phi(\sigma_U(x)\cdot g)=(x,g).$$
In the above equation, $\sigma_U(\pi(p))$ is used to identify the fibre above $\pi(p)=x$ to $G$ by mapping $\sigma_U(\pi(p))$ to $e$. 
Conversely, if $(\psi,U)$ is a local bundle chart, then $\sigma_U(x) = \psi^{-1}(x,e)$ is a local section. 
\end{proof}
Local sections of $L(TM)$ are closely related to the intuitive notion of moving frames used earlier. To see this, suppose that $\sigma_U$ is such a local section of $L(TM)$.  By definition of $L(TM)$, this is equivalent to a family $(u_x)_{x\in U}$ of linear maps $u_x \in GL(\mathbb{R}^n,T_xM)$. Such a family determines a basis of each $T_xM$: the image of the canonical basis of $\mathbb{R}^n$. It is clear that a moving frame is equivalent to such a family and therefore to a local section.

Now, if $(\phi,U)$ and $(\psi,V)$ are two local bundle charts with $U\cap V\neq \emptyset$ and we write $ \phi(p)=(\pi(p),s_U(p))$ and $\psi(p)=(\pi(p),s_V(p))$, then for each $x \in U\cap V$, the element $s_V(p)(s_U(p))^{-1} \in G$  is in fact independent of the choice of $p $ in the fibre above $x$, $\pi^{-1}(\{x\})$. Indeed, if $r=pg$ is another element in the fibre then:
\[s_V(r)s_U(r)^{-1}=s_V(pg)s_U(pg)^{-1}=s_V(p)g(s_U(p)g)^{-1}=s_V(p)s_U(p)^{-1}.\]
This leads to the following definition:
\begin{defi}
Using the same notation as above, the smooth map defined for each $x\in U\cap V$ by:
\[g_{VU}(x)=s_V(p)(s_U(p))^{-1},\] where $p\in \pi^{-1}(\{x\})$ is arbitrary, is called a \emph{transition function}.
\end{defi}  
The transition function describes how to change the local bundle chart. This can be seen through inspection of the map $\psi \circ \phi^{-1}$ on $(U\cap V)\times G$ given by:
\[\psi\circ\phi^{-1}(x,g)=(x,g_{VU}(x)g).\]
Indeed, for $p=\phi^{-1}(x,e)$, $g_{VU}(x)=s_V(\phi^{-1}(x,e))$ and: 
\[\psi\circ\phi^{-1}(x,g)=(x,s_V(\phi^{-1}(x,g)))=(x,s_V(\phi^{-1}(x,e)g))=(x,s_V(\phi^{-1}(x,e))g).\]
The transition functions satisfy the following properties:
\begin{prop}
\label{prop:transition}
\begin{equation}  g_{UU}=e, \quad g_{UV}=g_{VU}^{-1}, \quad g_{UV}g_{VW}g_{WU}=e.
\end{equation}
\end{prop}

It is in fact the case that the transition functions contain all of the information of the fibre bundle; the above properties guarantee that local bundle charts can be glued together appropriately. They are easily interpreted in terms of the local sections $\sigma_U$ and $\sigma_V$ determined by $(\phi,U)$ and $(\psi,V)$: on $U\cap V$, $\sigma_Ug_{UV}=\sigma_V$. On $L(TM)$, thinking of local sections as moving frames, $g_{UV}$ is just the change of basis matrix from $\sigma_U(x)$ to $\sigma_V(x)$. We can now reformulate our previous conclusions as follows: an affine connection on $L(TM)$ is equivalent to the data consisting of a matrix-valued differential form $\omega_U$ on each local bundle chart $(\phi,U)$ of $L(TM)$. On the intersection of any two local bundle charts $U$ et $V$, the forms $\omega_U$ and $\omega_V$ must satisfy:
\begin{equation}\label{chg_con_ex}\omega_V= (g_{UV}^*\theta)+ \mathfrak{ad}_{g_{UV}^{-1}}(\omega_U). \end{equation} 
This leads to the first definition of a connection on a principal fibre bundle:
\begin{defi}
\label{def:connexion_locale}
Let $(P,\pi,M)$ be a $G$-principal fibre bundle over $M$, a connection on $P$ is the data consisting of a differential form $\omega_U$ with values in the Lie algebra $\mathfrak{g}$ of $G$ for each local section $\sigma_U$ of $P$, such that if two local sections are related by $\sigma_V=\sigma_Ug_{UV}$ then:
%
\begin{equation}\omega_V= (g_{UV}^*\theta_G)+ \mathfrak{ad}_{g_{UV}^{-1}}(\omega_U), \end{equation}
where $\theta_G$ is the Maurer-Cartan form of $G$.
\end{defi}
\section{Vertical vectors}
The above definition is very useful for local computations on manifolds, and is used extensively in the Physics literature. However, from a conceptual perspective it is interesting to point out that these local connection forms actually stem from a global object defined on $P$. To see this we first need to study the projection map $\pi$ of a $G$-principal fibre bundle $(P,\pi,M)$ in more detail. 

According to Definition~\ref{def:fibreprincipal}, $\pi: P \rightarrow M$ is a smooth surjection.  In fact, $\pi$ is a submersion since, if $p\in P$, one can always find a local section $\sigma_U$ (cf. Proposition~\ref{prop:section_locale}), that satisfies $\sigma_U(\pi(p))=p$. Such a section is a differentiable right inverse of $\pi$ and the tangent map $d{\sigma_U}_x$ is a right inverse of $d\pi_{\sigma_U(x)}=d\pi_{p}$. Consequently, $(V_p)_{p\in P}$, where $V_p=\ker d\pi_p$ is a smooth distribution of $TP$. 

Elements of $V_p, p\in P$ will be referred to as \emph{vertical vectors}. Intuitively, they are the vectors in $T_pP$ that have no component in the direction of the basis. In other words, they are the tangent vectors to curves entirely contained in one of the fibres of $P$.

\begin{defi}
\label{def:champ_fondamental}
Denote the Lie algebra of $G$ by $\mathfrak{g}$ and let $A\in \mathfrak{g}$. $A$ gives rise to a vector field, called the \emph{fundamental field}, $A^*$, according to the formula:
\begin{equation} A^*_p = \left.\frac{\textrm{d}}{\textrm{d}t}(p\exp(At))\right|_{t=0}. \end{equation}
\end{defi}
For fixed $p$, $A^*_p$ is nothing more than the image of $A$ under the tangent map at $e$ of the map $\mathscr{L}_p: G\rightarrow P$, given by $\mathscr{L}_p(g)=pg.$ Hence, for fixed $p$,  $A \mapsto A^*_p$ is linear, and we claim that it is injective:
suppose that $A^*_p=0$ for some $A\in \mathfrak{g}$, and let $s\in \mathbb{R}$, then:
\[\begin{aligned}0=\left.\frac{\textrm{d}}{\textrm{d}t}\left(p\exp(tA)\exp(sA) \right)\right|_{t=0},&=\left.\frac{\textrm{d}}{\textrm{d}t}\left(p\exp((t+s)A)\right)\right|_{t=0}\\&=\left.\frac{\textrm{d}}{\textrm{d}t}\left(p\exp(tA) \right)\right|_{t=s}.\end{aligned}\]
It follows that $s\mapsto p\exp(sA)$ is the constant map $s\mapsto p$. Since the group $G$ acts freely on $P$ necessarily $\exp(sA)=e$ for every $s\in \mathbb{R}$. However, $\exp: \mathfrak{g} \rightarrow G$ is a local diffeomorphism near $0$, so $A=0$.
Last of all, $A^*_p\in V_p$ for each $p$, since: \[d\pi_p(A^*_p)=\left.\frac{\textrm{d}}{\textrm{d}t}(\pi(p\exp(At)))\right|_{t=0}=\left.\frac{\textrm{d}}{\textrm{d}t}\pi(p)\right|_{t=0}=0.\]
Consequently, this induces a vector space isomorphism $V_p \cong \mathfrak{g}$, and at each $p\in P$ we have the following short exact sequence:
%
\[0\rightarrow \mathfrak{g} \rightarrow T_pP \rightarrow T_{\pi(p)}M \rightarrow 0.\]
A local section $\sigma_U$ right splits the sequence:
%
\[0\rightarrow \mathfrak{g} \rightarrow T_{\sigma_U(x)}P \rightarrow T_xM \rightarrow 0,\]
so that we have the isomorphism: $T_{\sigma_U(x)}P \cong \mathfrak{g} \oplus T_xM.$


\section{Connection as a $\mathfrak{g}$-valued differential form on $P$}
\label{par:connexion_loc_vers_connexion_glob}
We can now introduce the second definition of a connection that we alluded to at the beginning of the preceding paragraph. To illustrate the construction, we return to the example of an affine connection; our arguments are, however, completely independent of this choice and can be applied to any connection as defined by Definition~\ref{def:connexion_locale}.

Suppose that we have a local connection form $\omega_U$ on each local bundle chart $(\phi,U)$ of $L(TM)$ and that they are compatible in the sense of~\eqref{chg_con_ex} on the intersection of any two charts. For any given chart $(\phi,U)$, let $\sigma_U$ denote the section of $L(TM)$ given by $\sigma_U(x)=\phi^{-1}(x,e)$. In light of the concluding remarks of the previous paragraph, for each $x\in U$ we define a linear map: $\omega_{\sigma_U(x)}:T_{\sigma_U(x)}L(M) \rightarrow M_n(\mathbb{R})$ by:
\begin{equation} \omega_{\sigma_U(x)}(d{\sigma_U}_x(Y) + A^*_{\sigma_U(x)} )= {\omega_U}_{x}(Y) + A, \,\, Y \in T_xM.  \end{equation}
We then extend the definition to other points in the fiber above $x$ by imposing the equivariance:
\begin{equation} \label{eq:equivarianceadroite} R_g^*\omega = \frak{ad}_{g^{-1}}\omega, \end{equation}
where $R_g$ is the smooth map $p \mapsto pg.$ This means that for any $p\in \pi^{-1}(\{x\}), g\in GL_n(\mathbb{R})$:
%
\begin{equation} \omega_{pg}(dR_g(X))= \mathfrak{ad}_{g^{-1}}\omega_{p}(X), \,\, X\in T_pP. \end{equation}
In this way we get a smooth matrix valued differential form on the bundle $\pi^{-1}(U)$, that, additionally, satisfies: \begin{equation} \label{eq:connexion_fundamental_field} \omega(A^*)=A. \end{equation}
This can be seen in the following manner. Let $p\in \pi^{-1}(U)$ and set $x=\pi(p)$. One can find $g\in GL_n(\mathbb{R})$ such that $p=\sigma_U(x)g$, hence:
\[\omega_p(A^*_p)=\mathfrak{ad}_{g^{-1}}\omega_{\sigma_U(x)}(d{R_{g^{-1}}}_{p}(A^*_p)).\]
Moreover, for any $A\in \mathfrak{g}$: 
\[\begin{aligned} d{R_{g^{-1}}}_{p}(A^*p)=\left.\frac{\textrm{d}}{\textrm{d}t}\left(p\exp(At)g^{-1} \right)\right|_{t=0}&=
\left.\frac{\textrm{d}}{\textrm{d}t}\left(pg^{-1}g\exp(At)g^{-1} \right)\right|_{t=0},\\&=\left.\frac{\textrm{d}}{\textrm{d}t}\left(pg^{-1}\exp(\mathfrak{ad}_gAt) \right)\right|_{t=0},\\&= (\mathfrak{ad}_g A)^*_{\sigma_U(x)}. \end{aligned}\]
Consequently: $\omega_p(A^*_p)=\mathfrak{ad}_{g^{-1}}\mathfrak{ad}_gA=A.$

In order to complete the construction of a differential form on $L(TM)$, it remains to show that the definition is consistent on the intersection of any two bundle charts $U,V$. Let $(\phi,U)$ and $(\psi,V)$ be two local bundle charts and denote by $\sigma_U$, $\sigma_V$ the associated local sections. Finally, we call $\omega^U$ and $\omega^V$ the forms on $\pi^{-1}(U)$ and $\pi^{-1}(V)$ respectively, constructed as described above from local connection forms $\omega_U$ and $\omega_V$ on $U$ and $V$ respectively.

The invariance~\eqref{eq:equivarianceadroite} implies that it is sufficient to check that for $x\in U\cap V$: $\omega^V_{\sigma_V(x)}=\omega^U_{\sigma_V(x)}$. Additionally,~\eqref{eq:connexion_fundamental_field} implies that we only need to show that for any vector field $Y\in T_xM$: \[\omega^{V}_{\sigma_V(x)}(d{\sigma_V}_x(Y))=\omega^{U}_{\sigma_V(x)}(d{\sigma_V}_x(Y)).\]
Let us evaluate the right-hand side:
\begin{equation*}\begin{aligned} \omega^{U}_{\sigma_V(x)}(d{\sigma_V}_x(Y))&=\omega^{U}_{\sigma_U(x)g_{UV}(x)}(d(\sigma_Ug_{UV})_x(Y)) ,\\&\hspace{-1.7cm}= \omega^{U}_{\sigma_U(x)g_{UV}(x)}\left(d{\mathscr{L}_{\sigma_U(x)}}_{g_{UV(x)}}(d{g_{UV}}_x(Y))+d{R_{g_{UV}(x)}}_x(d{\sigma_U}_x(Y))\right)\!\!, \\&\hspace{-2.7cm}=\mathfrak{ad}_{g_{UV}(x)^{-1}}\omega^{U}_{\sigma_U(x)}(d{\sigma_U}_x(Y))+ \omega^{U}_{\sigma_U(x)g_{UV}(x)}\left(d{\mathscr{L}_{\sigma_U(x)}}_{g_{UV(x)}}(d{g_{UV}}_x(Y))\right)\!\!.\end{aligned} \end{equation*} 
In the last two lines we recall that $\mathscr{L}_p, p\in L(TM)$ is defined by: $g\mapsto pg$. Let us focus our attention on the second term of the final equation. Choose a curve $\gamma$ on $M$ such that $\gamma(0)=x$ and $\dot{\gamma}(0)=Y$, and note that:
\begin{equation}
\begin{aligned}
d{\mathscr{L}_{\sigma_U(x)}}_{g_{UV(x)}}(d{g_{UV}}_x(Y))&=\left.\frac{\textrm{d}}{\textrm{d}t}\left(\sigma_U(x)g_{UV}(\gamma(t))\right) \right|_{t=0}
,\\&=\left.\frac{\textrm{d}}{\textrm{d}t}\left(\sigma_V(x)g_{UV}(x)^{-1}g_{UV}(\gamma(t))\right) \right|_{t=0}.
\end{aligned}
\end{equation}
From the final equation we see the left-hand side is actually a tangent vector to a curve in the fibre of $L(M)$ containing $\sigma_V(x)$; in other words it is a vertical vector field. To determine to which element $A \in \mathfrak{gl_n(\mathbb{R})}$ it corresponds, we only need to calculate the derivative at $0$ of the curve in $GL_n(\mathbb{R})$ given by $t\mapsto g_{UV}(x)^{-1}g_{UV}(\gamma(t))$. The result is:
$d{L_{g_{UV}(x)^{-1}}}_{g_{UV}(x)}(d{g_{UV}}_x(Y))=(g_{UV}^*\theta)_x(Y)$. Therefore, using~\eqref{chg_con_ex}:
%
\begin{equation}
\begin{aligned}
\omega^{U}_{\sigma_V(x)}(d{\sigma_V}_x(Y))&=\mathfrak{ad}_{g_{UV}(x)^{-1}}{\omega_{U}}_x(Y)+(g_{UV}^*\theta)_x(Y),
\\&= {\omega_V}_x(Y).
\end{aligned}
 \end{equation}
Since $\omega^{U}$ et $\omega^V$ coincide on their common domain of definition, we have thus shown that they can be glued together to yield a matrix valued differential form on $L(TM)$. This leads to the following definition:
\begin{defi}
\label{def:connexion_principale}
Let $(P,G,\pi,M)$ be a smooth principal fibre bundle. A connection on $P$ is a smooth $\mathfrak{g}$-valued differential form $\omega$ that satisfies:
\begin{enumerate}
\item $\omega(A^*)=A$,
\item $R_g^*\omega=\mathfrak{ad}_{g^{-1}}\omega.$
\end{enumerate}
\end{defi}
As remarked above, our previous computations generalise without essential modification to the case of an arbitrary Lie group $G$ with Lie algebra $\mathfrak{g}$. Furthermore, they are the hard part of the proof that Definition~\ref{def:connexion_principale} is equivalent to Definition~\ref{def:connexion_locale}. To obtain $\omega_U$ from $\omega$, it suffices to pullback along the local section $\sigma_U$ \footnote{This is quite natural given the short exact sequences at the end our discussion on vertical vectors.}: $\omega_U=\sigma_U^*\omega$.

\section{Principal connection as a $G$-equivariant horizontal distribution} 
To close this discussion on principal connections, we would like to mention that there is a third equivalent definition, which is conceptually useful:
%
\begin{defi}
A principal connection on principal fibre bundle $(P,G,\pi,M)$ is a smooth $G$-equivariant distribution complementary to the vertical vector distribution i.e. a family of vector subspaces $(H_p)_{p\in P}, H_p \subset T_pP$ such that for any $p\in P, g\in G$.
\begin{enumerate} \item  $T_pP = H_p \oplus V_p,$
\item $(dR_g)(H_p)=H_{pg}.$ (equivariance)
\item The association $p\mapsto H_p$ is smooth in the sense that on a neighbourhood of any point $p\in P$ one can find $n$ vector fields that generate $H_q$ at each point $q$ in the neighbourhood.
\end{enumerate}
\end{defi} 
For a proof of the equivalence with our previous definitions, we refer the reader to~\cite{Naber:2010aa,Bleeker:2005aa}.
\newpage
\section{Associated bundles}\label{sec:fibre_associe}
In the main text we will tend to think of principal bundles as general frame bundles. The following construction further justifies this point of view and is used repeatedly in the text.

To introduce our point of view, let us borrow, as we often do, a situation from Physics. Imagine that we would like to describe the movement of a particle in Newton's absolute space. To do this, we set up a frame of reference and a system of cartesian coordinates $(x,y,z)$. With respect to this frame of reference, we measure a certain number of physical quantities, of different nature such as the position, velocity or angular momentum, associated with the movement of the particule. These quantities can each be represented as one or a collection of real numbers. It is natural to ask, how can we compare our measurements with those carried out in another frame of reference ? Do these numbers change, and if so, how ? To simplify things a little, assume that the reference frames are anchored in the same point so that the transformation group is simply the familiar group of rotations $SO(3)$. In this situation, we will find that if we rotate our frame using $A\in SO(3)$, then the 3 real numbers that describe the velocity $(v_i)_{i\in \{1,2,3\}}$ change according to the following rule: $\tilde{v}^i=(A^{-1})^i_jv^j$. In view of this, we will say that the velocity is a \enquote{vector} quantity; similarly, the mass, which will not change, will be said to be a \enquote{scalar} quantity. In other words, we classify quantities according to the representation of the rotation group to which they correspond.

In General Relativity, tensor quantities of this type are still used to describe systems, the difference being that the transformation group applies to local frames. The machinery that we are now going to describe, enables us to construct a vector bundle over a manifold $M$, given any $G$-principal fibre bundle over $M$ - which contains the information about local frames - and a linear representation $(V,\rho)$ of the group $G$. We will denote this vector bundle by $P\times_G V$, the fiber above any point of this bundle is a vector space of quantities with the transformation rule prescribed by the representation. More generally, an adaptation of our discussion enables the definition of associated bundles $P\times_G X$ for a number of differentiable actions of the group $G$ on a manifold $X$.


\section{Constructing an associated vector bundle}
Let $(P,G,\pi,M)$ be a $G$-principal bundle over $M$ and $(V,\rho)$ a smooth finite dimensional linear representation (to simplify: $V\approx \mathbb{K}^n, \mathbb{K}=\mathbb{R},\mathbb{C}$ ) of $G$.
The construction of $P\times_{G}V$ is largely inspired by our usual experience of tensor fields.  Consider the product manifold $P\times V$ and the smooth left action of $G$ on $P\times V$ given by:
\begin{equation} \begin{array}{ccc} G \times (P\times V) &\longrightarrow& P \times V \\ (g,(r,v)) &\longmapsto& (rg,\rho(g)^{-1}v).  \end{array} \label{action_G} \end{equation} $P\times_G V$ is simply defined as the quotient space $(P \times V)/G$. 

To motivate this choice, it is illuminating to think of a pair $(r,v)$ as the data consisting of a local frame $r$ and the coordinates of a vector $v$ in that frame. Multiplying from the right a frame by an element $g\in G$ corresponds to changing frame ($g$ is the change of basis matrix) and, accordingly, the components of the vector $v$ should change according to the usual change of basis rule in linear algebra.

The proof of the fact that $P\times_G V$ is a vector bundle over $M$ with fibre $V$ is often left as an exercise in the literature. For the benefit of impatient readers, we sketch the proof below. To simplify notations a little we introduce the notation $E=P\times_G V$.
Let \hbox{$\textsf{p}: P\times V \longrightarrow P\times_G V$} be the canonical projection.
Let $(\phi, U)$ be a local bundle chart and suppose that $p\in U, \phi(p)=(\pi(p),s_u(p))$. Shrinking, if necessary, $U$ we can assume that it is the defining domain of a local chart $(x,U)$ on $M$. 
Set now: \begin{equation*}  \begin{array}{cccc}\overline{x}:  &\pi^{-1}(U) \times V &\longrightarrow& x(U) \times V  \\ &(r,v) &\longmapsto& (x(\pi(r)), \rho(s_u(r))v). \end {array} \end{equation*}
Observe that it factors to a map: $\tilde{\bar{x}}: \textsf{p}(\pi^{-1}(U)\times V) \longrightarrow x(U)\times V$. Indeed, if $(r,v) \sim (r',v')$ then one can find $g \in G$ such that  $r'=rg$ and $v'=\rho(g)^{-1}v$. Hence: \begin{equation*} \left\{\begin{array}{l} x(\pi(r'))=x(\pi(rg))=x(\pi(r)), \\  \begin{aligned}\rho(s_u(r'))v'=\rho(s_u(rg))\rho(g^{-1})v&=\rho(s_u(r)g) \rho(g)^{-1}v,\\&= \rho(s_u(r))\rho(g)\rho(g)^{-1}v,\\& = \rho(s_u(r))v. \end{aligned}\end{array}\right.\end{equation*}
We will now show that the maps $\tilde{\bar{x}}$ are a bundle atlas for $E$. This relies on two lemmata:
\begin{lemm}
Let $G$ be a topological group and $(X,\mathscr{T})$ a topological space on which $G$ acts continuously from the left, i.e. the map $ (g,x) \mapsto g\cdot x $ is continuous for the product topology. In this case, if $O$ is an open set in $X$ and $A \subset G$, then the set $A\cdot O= \left\{ a \cdot x, a\in A, x\in O \right\}$ is open.
\end{lemm}
\begin{proof} For any fixed $g\in G$, the map $x\mapsto g\cdot x$ is a homeomorphism with inverse $x\mapsto g^{-1} \cdot x$; in particular it is an open map. Hence, $g\cdot O$ is open. The result follows for an arbitrary subset $A\subset G$ by an arbitrary union of open sets. \end{proof}
\begin{lemm}
The canonical projection map $\textsf{p}$ is open.
\end{lemm}
\begin{proof}
Let $O$ be an open subset of $P\times V$. By definition of the quotient topology the set $\textsf{p}(O)$ is open if and only if  $\textsf{p}^{-1}(\textsf{p}(O))$ is open, but:
\begin{align*} \textsf{p}^{-1}(\textsf{p}(O))&=\left\{ (r,v) \in P\times V, \textsf{p}(r,v)\in \textsf{p}(O) \right\} ,\\ &=  \left\{(r,v)\in P\times V, \exists (r',v') \in O , \textsf{p}(r,v)=\textsf{p}(r',v') \right\} ,\\ &\hspace{-1mm}=\left\{  (r,v) \in P\times V, \exists (r',v')\in O, \exists g \in G, (r,g)\!=\!(r'g,\rho(g)^{-1}v)\!\right\}\!\!,\\ &= g\cdot O.\end{align*}
Since the action defined by~\eqref{action_G} is continuous, we conclude by the previous Lemma.
\end{proof}
It follows that the defining domain of $\tilde{\bar{x}}$, $\textsf{p}(\pi^{-1}(U)\times V)$, is an open subset of $E$. Define now the surjective map: $$ \begin{array}{cccc}\bar{\pi}: &P\times V &\longrightarrow& M \\& (p,v) &\longmapsto& \pi(p), \end{array}$$ which factors, like $\bar{x}$, to a surjective map: $\tilde{\bar{\pi}}: E \longrightarrow M$. Moreover:
\[\bar{\pi}^{-1}(U)=\textsf{p}^{-1}(\tilde{\bar{\pi}}^{-1}(U)).\]
Therefore, since $\textsf{p}$ is surjective, one has:
\[\textsf{p}(\bar{\pi}^{-1}(U))=\tilde{\bar{\pi}}^{-1}(U),\] 
furthermore, $\bar{\pi}^{-1}(U)=\pi^{-1}(U)\times V$, thus:
\[\tilde{\bar{\pi}}^{-1}(U)=\textsf{p}(\pi^{-1}(U)\times V).\footnote{\textrm{This is actually sufficient to prove that it is open}.}\]
Overall: $\tilde{\bar{x}}: \tilde{\bar{\pi}}^{-1}(U) \longrightarrow x(U)\times V \subset \mathbb{R}^n \times V$.
To show that $\tilde{\bar{x}}$ is itself a homeomorphism, we describe explicitly its inverse. Choose an arbitrary element $g\in G$ and set:
\begin{equation} \phi: \begin{array}{ccc} x(U)\times V &\longrightarrow& \tilde{\bar{\pi}}^{-1}(U)=p(\pi^{-1}(U)\times V) \\ (a,b) &\longmapsto& \textsf{p}(\phi^{-1}(x^{-1}(a),g),\rho(g)^{-1}\cdot b)).\end{array} \end{equation}
As a composition of continuous functions, $\phi$ is continuous and is actually independent of the choice of $g$ \footnote{It would have been simpler to take directly $g=e$.}. Moreover:
\[\begin{aligned} \phi(\tilde{\bar{x}}(p(r,v)))&=\phi((x(\pi(r)),\rho(s_u(r))v)),\\&=p(\phi^{-1}(\pi(r),g),\rho(g)^{-1}\rho(s_u(r))v)).\end{aligned}\]
Define $r'=\phi^{-1}(\pi(r),g)$, clearly: $r'\in \pi^{-1}(\pi(r))$ so $r'$ and $r$ are in the same orbit, hence we can find $g'\in G$ satisfying $r'=rg'$ i.e.  $r=r'g'^{-1}$.
By consequence:
\begin{align*} \textsf{p}(\phi^{-1}(\pi(r),g),\rho(g)^{-1}\rho(s_u(r))v)) &= \textsf{p}(r',\rho(g)^{-1} \rho(s_u(r'g'^{-1})v) \\& =\textsf{p}(rg',\rho(g)^{-1} \rho(\underbrace{s_u(r')}_{g})\rho(g'^{-1})v),\\&=\textsf{p}(rg',\rho(g')^{-1}v). \end{align*}
Hence: \[\phi(\tilde{\bar{x}}(\textsf{p}(r,v)))=p(rg',\rho(g')^{-1}v)=\textsf{p}(r,v),\] 
and $\phi$ is a right inverse of $\tilde{\bar{x}}$.
Let us compute now $\tilde{\bar{x}}(\phi(a,b))$:
\begin{align*}\tilde{\bar{x}}(\phi(a,b)) &=\tilde{\bar{x}}(\textsf{p}(\phi^{-1}(x^{-1}(a),g),\rho(g)^{-1} b)),\\&= \bar{x}(\phi^{-1}(x^{-1}(a),g),\rho(g)^{-1} b),\\&=(a, \rho(g) \rho(g)^{-1}b)=(a,b). \end{align*}
Consequently, $\phi$ is the inverse map to $\tilde{\bar{x}}$, which is a homeomorphism. If we consider the maximal atlas containing all charts constructed in this manner, it is not difficult to see that this is a smooth structure for $E$ which is hence a smooth manifold of dimension $\dim M + \dim V$. Furthermore, studying the form of these charts, one can see that $E$ is a vector bundle over $M$ with model fibre $V$. For instance, a fibre $V_q=\tilde{\bar{\pi}}^{-1}(\{x\})=\textsf{p}(\bar{\pi}^{-1}(\{q\}))=\textsf{p}(\pi^{-1}(\{q\})\times V), q\in M$ is naturally equipped with a vector space structure induced by that of  $\{r\}\times V$ for each $r\in \pi^{-1}(\{x\})$. Indeed, if $\mathfrak{v}_1=\textsf{p}(r,v)$ and $\mathfrak{v}_2=\textsf{p}(r',v')$ are two elements of $V_q$, then, since $r'\in \pi^{-1}(\{\pi(r)\}=\{q\})$, one can find $g\in G$ such that $r=r'g$. In particular: $\mathfrak{v}_2=(r,\rho(g)^{-1}v')$. Consequently we set: \[\mathfrak{v}_1+\mathfrak{v}_2=\textsf{p}((r,v)+(r,\rho(g)^{-1}v'))=\textsf{p}(r,v+\rho(g)^{-1}v'),\] this is independent of the choice of representative and so we have a well-defined addition $+$. Analogously, if $\lambda \in \mathbb{K}$, we set:
\[\lambda\cdot \mathfrak{v}_1=\textsf{p}(\lambda\cdot (r,v))=\textsf{p}((r,\lambda v)).\]
Once more, linearity of the representation can be used to show that this definition is independent of the choice of $(r, v)$ in the class $\textsf{p}(r,v)$: \[\textsf{p}((r,\lambda v))=\textsf{p}(rg, \rho(g)^{-1}(\lambda v))= \textsf{p}(rg, \lambda \rho(g)^{-1}v).\] This linear structure is chosen so that $ \tilde{\phi}_q= \tilde{\bar{x}}_{|\tilde{\bar{\pi}}^{-1}(\{q\})}: V_q \longrightarrow \{x(q)\} \times V$ becomes a vector space isomorphism:
\begin{align*} \tilde{\phi}_q(\lambda\mathfrak{v}_1 + \mu\mathfrak{v}_2) =\tilde{\bar{x}}(\textsf{p}(r,\lambda v_1+\mu v_2))&=(x(q), \rho(s_u(r))(\lambda v_1+ \mu v_2)),\\&\hspace{-.2cm}=(x(q),\lambda \rho(s_u(r)).v_1+\mu\rho(s_u(r))v_2)),\\&\hspace{-1.2cm}= \lambda(x(q), \rho(s_u(r)).v_1) +\mu(x(q),\rho(s_u(r))v_2),\\&\hspace{-1cm}=\lambda\tilde{\phi}_q(\mathfrak{v}_1)+\mu\tilde{\phi}_q(\mathfrak{v}_2); \quad \lambda,\mu \in \mathbb{K}, \mathfrak{v}_i \in V_q.  \end{align*}
We omit the proof that the action is proper which implies that $P\times_G V$ is indeed Hausdorff.
%% 
\section{Examples of associated bundles}
\label{par:fibreassocie}
We will now give some examples of associated bundles, the first of which are the usual tangent and cotangent bundles $TM$ et $T^*M$:
\begin{enumerate}
\item $TM$ is the associated bundle to $L(TM)$ corresponding to the fundamental representation of $GL_n(\mathbb{R})$,
\item $T^*M$ is the associated bundle $L(TM)$ corresponding to the dual or contragredient representation: $P\mapsto {}^{t}P^{-1}$,
\item more generally, the bundle of tensors of type $(p,q)$ is the associated bundle to $L(TM)$ corresponding to the representation $(\rho, \otimes^{p+q}\mathbb{R}^n)$, defined by: \[\rho(P)v_1\otimes\dots\otimes v_p \otimes l^1\otimes\dots\otimes l^q\!=\!(Pv_1)\otimes \dots \otimes (Pv_p) \otimes ({}^tP^{-1}l^1)\otimes\dots\otimes({}^tP^{-1}l^q).\]
\end{enumerate}
%The following example is important for Chapter~\ref{chapter:projective}, so we present it as a definition: 
%\begin{defi}
%\label{def:densites}
%Let $\omega \in \mathbb{C}$, a projective density of weight $\omega$\footnote{We may also speak of densities of projective weight $\omega$} is a smooth section of the bundle $\mathcal{E}(\omega)$ associated to $L(TM)$ with the representation of $GL_n(\mathbb{R})$ on $\mathbb{R}$ given by:
%\[\begin{array}{rcl} GL_n(\mathbb{R})\times \mathbb{R} &\longrightarrow& \mathbb{R} \\ (A,v) &\longmapsto & |\det A|^\frac{\omega}{n+1}v. \end{array}\]
%If $\mathscr{B}$ is any fibre bundle on $M$, we will write $\mathscr{B}(\omega)$ for $\mathscr{B}\otimes\mathcal{E}(\omega)$.
%\end{defi}
%Note that $\mathcal{E}(\omega)$ is a trivial line bundle; one can construct a non-zero global section using a partition of unity.

\section{Covariant derivative on an associated vector bundle}
\label{sec:derivee_fibreassocie}
A principal connection $\omega$ on a principal fibre bundle $(P,G,\pi,M)$ induces an affine connection in the sense of Definition~\ref{def:connexion_carmo} on any associated vector bundle. In Physics literature this is often referred to as a covariant derivative. The following definition will help us simplify the construction:
\begin{defi}
\label{def:morphism_fibre_principaux}
Let $(P,G,\pi)$ and $(P',G',\pi')$ be two fibre bundles over $M$ and $\phi: P \rightarrow P'$ be a smooth map. $\phi$ is a principal bundle morphism if:
\begin{enumerate}
\item there is a group homomorphism $\varphi: G \rightarrow G'$ such that for any $p\in P,g\in G$: \[\phi(pg)=\phi(p)\varphi(g),\]
\item the following diagram is commutative:
\[
  \begin{tikzcd}[column sep=small]
    P \arrow[swap]{dr}{\pi} \arrow{rr}{\phi}  && P' \arrow{dl}{\pi'} \\
      &M&
  \end{tikzcd}.
\]
\end{enumerate}
\end{defi}
Presently, an interesting example is given by the following lemma:
\begin{lemm}
Let $(P,G,\pi,M)$ be a principal fibre bundle and $P\times_G V$ an associated vector bundle corresponding to a representation $(V,\rho)$ of $G$. In this case, there is a principal bundle morphism $P \longrightarrow L(P\times_GV)$ where $L(P\times_G V)$ is the frame bundle of $P\times_G V$ (cf. Paragraph~\ref{fibrereperes}) given by:
%
\begin{equation}
 \begin{array}{crcl}\Phi:&P &\longrightarrow & L(P\times_G V) \\ &r &\longmapsto& (\pi(r), u_r). \end{array}
\end{equation}
In the above, $u_r \in GL(V,(P\times_G V)_{\pi(r)})$ is defined by $ v \mapsto p(r,v)$ and $p$ is the canonical projection from $P\times V$ onto $P\times_G V.$ 
\end{lemm}
\begin{proof}
We simply check that: $\Phi(rg)=\Phi(r)\rho(g)$; for which it is sufficient to show that $u_{rg}=u_r \circ \rho(g)$. For each $r\in P, g\in G$: $u_{rg}(v)=p(rg,v)=p(r,\rho(g)v)=u_r(\rho(g)(v))$.
\end{proof}
It follows that a local section $\sigma_U$ of $P$, gives rise to a local section of $L(P\times_GV)$ according to the formula $\tilde{\sigma}_U= \Phi\circ\sigma_U$. Furthermore, the tangent map to the representation morphism $\rho$ at the identity of $G$ induces a Lie algebra representation of $\mathfrak{g}$ that we will call $\rho_*$. The local connection form $\omega_U=\sigma_U^*\omega$ induces a local connection form on $L(P\times_G V)$ according to: $\tilde{\omega}_U=\rho_*\omega_U$. 

To convince ourselves that this is indeed a connection, let us verify that~\eqref{chg_con_ex} holds for $\tilde{\omega}$. Let $\sigma_V$ be another local section such that $U\cap V\neq \emptyset$. Since $\Phi$ is a principal fibre bundle morphism, $\tilde{\sigma}_V=\Phi(\sigma_Ug_{UV})=\Phi(\sigma_U)\rho(g_{UV})$ and:
 %
\[\tilde{\omega}_V=\rho_* \omega_V =\rho_*(g_{UV}^*\theta) + \rho_*\mathfrak{ad}_{g_{UV}^{-1}}(\omega_U).\]
The result follows from:
\[\begin{aligned} \rho_*\mathfrak{ad}_{g_{UV}^{-1}}(\omega_U)&= d\rho_e \circ d(Ad_{g_{UV}^{-1}})_e(\omega_U), \\ &=d(\rho \circ Ad_{g_{UV}^{-1}})_e(\omega_U),\\&=d(Ad_{\rho(g_{UV})^{-1}}\circ \rho)_e(\omega_U)=\mathfrak{ad}_{\rho(g_{UV})^{-1}}(\tilde{\omega}_U),\end{aligned}\]
and:
\[\begin{aligned} \rho_*g_{UV}^*\theta&=d\rho_e \circ d{L_{g_{UV}^{-1}}}_{g_{UV}}(dg_{UV}),\\
&= d(\rho \circ L_{g_{UV}^{-1}})_{g_{UV}}(dg_{UV}),\\&=d{L_{\rho(g_{UV})^{-1}}}_{\rho(g_{UV})}(d\rho_{g_{UV}}\circ dg_{UV}),\\&=d{L_{\rho(g_{UV})^{-1}}}_{\rho(g_{UV})}(d\rho(g_{UV})).\end{aligned}\]

\section{Fibre bundle reductions and geometric properties }
The final topic that we wish to touch upon briefly in this walkthrough on Principal fibre bundles is that of fibre bundle reductions. Our interest in this is mainly conceptual: orientation or metric tensors can be reinterpreted as reductions of $L(M)$ to an $H$-principal fibre bundle where $H\subset GL_n(\mathbb{R})$ is a closed subgroup.

\begin{defi} Let $H$ be a closed subgroup of a Lie group $G$, $(P,\pi,M)$ a $G$-principal fibre bundle and $\iota: H \rightarrow G$ the canonical injection. A reduction of $P$ is a $H$-principal fibre bundle  $(P',\pi',M)$ and a principal bundle morphism $\phi$ such that: $\phi(qh)=\phi(q)\iota(h), q \in P', h\in H$. 
In this case: $\phi$ is an immersion and we have the isomorphism $P'\times_H G \cong P$ where $H$ acts on $G$ by left multiplication.
\end{defi}

The existence of a reduction is generally subject to topological constraints. For instance, if $G=GL_n(\mathbb{R})$, $H=\{\textrm{Id}\}$ and $P=L(TM)$  then there is a reduction $P'$ if and only if $M$ is parallelisable. In a similar fashion, if $H=GL_n(\mathbb{R})^+$, the subgroup of matrices with positive determinant, then the existence of a reduction is equivalent to orientability. This is more easily seen when thinking in terms of an orientation atlas:  one can construct the bundle $P'$ by imitating the method described in Appendix~\ref{fibrereperes} but restricting to positively oriented frames: the orientation atlas is exactly what is needed to guarantee that this is possible. In terms of transition functions, a reduction translates to the possibility to restrict their values to a subgroup. Finally, a choice of metric is equally equivalent to a reduction of the frame bundle which restricts to orthonormal frames: one can choose a covering such that the transition functions take their values in $O(p,q)$. If furthermore $M$ is orientable, one can work with positively oriented orthonormal frames.


==> annexe/transfo_connexion.tex <==
% !TEX root = ../smf_proj.tex
\chapter{The transformation law for $(\Omega^{i}_{j}(\cdot,e_i))$}
\label{annexe:transfo}
We follow the notation introduced in Section~\ref{sec:inv_diff_thomas}. Recall that in the equation:
\[\Omega_U= d\Pi_U + \Pi_U\wedge \Pi_U,\]
$\wedge$ is the matrix product where component-wise multiplication is replaced with the exterior product of differential forms and $d\Pi$ is the matrix $(d\Pi)^i_j = d(\Pi^i_j)$. 
We recall also that the transformation law for $\Pi_U$ is given by~\eqref{eq:transfo_pi}~:
\begin{equation}\Pi_V = g^{-1}dg + g^{-1}\Pi_Ug -\frac{1}{n+1}\textrm{tr}(g^{-1}dg)I_n - \frac{1}{n+1}g^{-1}Ag, \end{equation}
where $A^i_j=\textrm{tr}(g^{-1}dg(e_j))\omega^i$ and the local sections are related by $\sigma_V=\sigma_U g$ for some $g: U\cap V \rightarrow GL_n(\mathbb{R})$. 

To determine the transformation law for $(\Omega^{i}_{j}(\cdot,e_i))$ we first compute $\Omega_V$ in several steps. First of all, $d\Pi_V$~:
\begin{equation}
\label{eq:an_step1}
\begin{aligned}
d\Pi_V=&-\underline{g^{-1}\dd g g^{-1}\wedge \dd g} -\underline{g^{-1}\dd g g^{-1}\wedge\Pi_Ug} + g^{-1}d\Pi_U g-\underline{g^{-1}\Pi\wedge \dd g}\\ &+\frac{1}{n+1}\textrm{tr}(g^{-1}\dd g g^{-1}\wedge \dd g)I +\underline{\frac{1}{n+1}g^{-1}\dd g g^{-1}\wedge Ag} \\&- \frac{1}{n+1}g^{-1}\dd Ag + \underline{\frac{1}{n+1}g^{-1}A\wedge \dd g}.
\end{aligned}
\end{equation}
\noindent Followed by~:
\begin{equation} 
\label{eq:an_step2}
\begin{split}
\Pi_V\wedge \Pi_V=g^{-1}\Pi_U\wedge\Pi_U g + \underline{g^{-1}\Pi_U \wedge dg} -\uwave{\frac{1}{n+1}g^{-1}\Pi_U g \wedge \textrm{tr}(g^{-1}dg)I}\\-\frac{1}{n+1}g^{-1}(\Pi_U\wedge A)g +\underline{g^{-1}dg\wedge g^{-1}\Pi_U g} +\underline{g^{-1}dg\wedge g^{-1}dg}\\ -\uwave{\frac{1}{n+1}g^{-1}dg\wedge\textrm{tr}(g^{-1}dg)I}-\underline{\frac{1}{n+1}g^{-1}dgg^{-1}Ag} \\-\uwave{\frac{1}{n+1}\textrm{tr}(g^{-1}dg)I\wedge g^{-1}\Pi_U g}\\ - \uwave{\frac{1}{n+1}\textrm{tr}(g^{-1}dg)I\wedge g^{-1}\textrm{dg}}\\+\frac{1}{(n+1)^2}\underbrace{\textrm{tr}(g^{-1}dg)\wedge\textrm{tr}(g^{-1}dg))}_{=0}I\\+\uwave{\frac{1}{(n+1)^2}\textrm{tr}(g^{-1}\textrm{dg})I\wedge g^{-1}Ag} \\-\frac{1}{n+1}g^{-1}A\wedge \Pi_U g - \underline{\frac{1}{n+1}g^{-1}A\wedge dg}\\+\frac{1}{(n+1)^2}g^{-1}(A\wedge A)g+\uwave{\frac{1}{(n+1)^2}g^{-1}Ag\wedge \textrm{tr}(g^{-1}dg)I} 
\end{split}
\end{equation}
When we sum together~\eqref{eq:an_step1} and~\eqref{eq:an_step2}, the terms in~\eqref{eq:an_step2} underlined by a straight line cancel exactly those in~\eqref{eq:an_step1}. The terms in~\eqref{eq:an_step2} underlined with a wavy line cancel between themselves by anti-symmetry of the usual exterior product because $I$ commutes with any matrix. After simplification, we find that~:
\begin{equation}\label{eq:ann_step3} \begin{split} \Omega_V = g^{-1}\Omega_U g +\frac{1}{n+1}\textrm{tr}(g^{-1}dgg^{-1}\wedge dg)I -\frac{1}{n+1}g^{-1}dAg \\-\frac{1}{n+1}g^{-1}(\Pi_U\wedge A)g -\frac{1}{n+1}g^{-1}(A\wedge \Pi_U)g \\+\frac{1}{(n+1)^2}g^{-1}(A\wedge A)g. \end{split} \end{equation} 
Now, denote by $(\tilde{e}_i)$ the moving frame associated with $\sigma_V$, then, for each $i$, $\tilde{e}_i=g^k_i e_k$. Consequently, calling the components of $\Omega_V$, $\tilde{\Omega}^i_j$~:
\[\tilde{\Omega}^i_j(\cdot,\tilde{e}_i)=g^k_i\tilde{\Omega}^i_j(\cdot,e_k)=(g\Omega_V)^k_j(\cdot,e_k).\] Therefore, we only need to multiply~\eqref{eq:ann_step3} by $g$ and evaluate the trace in the basis $(e_i)$. Computing each term separately~:
\begin{equation}
\label{eq:ann_step4}
\begin{aligned}
(A\wedge \Pi_U)^k_j(\cdot,e_k)&=\sum_k \sum_m\textrm{tr}(g^{-1}dg(e_m))\omega^k\wedge \Pi^m_j(\cdot,e_k),
\\&=\sum_k\sum_m \textrm{tr}(g^{-1}dg(e_m))\sum_i \Pi^m_{\,\,j}(e_i) \omega^k\wedge \omega^i(\cdot,e_k),
\\&=\sum_k\sum_m \textrm{tr}(g^{-1}dg(e_m))\sum_i \Pi^m_{\,\,j}(e_i)(\delta^i_k\omega^k - \omega^i)),
\\&=-(n-1)\sum_m\Pi^m_j \textrm{tr}(g^{-1}dg(e_m)),
\\&=-(n-1) (\gamma'\Pi_U)_j.
\end{aligned}
\end{equation}
\noindent Similarly~:
\begin{equation}
\label{eq:ann_step5}
\begin{gathered}
(\Pi_U\wedge A)^k_j(\cdot,e_k)=-\textrm{tr}(g^{-1}dg(e_j))\sum_m\sum_k \Pi^k_m(e_k)\omega^m,\\
\begin{aligned}
(A\wedge A)^k_j(\cdot,e_k)&=-(n-1)\textrm{tr}(g^{-1}dg(e_j))\textrm{tr}(g^{-1}dg),
\\&=-(n-1)\textrm{tr}(g^{-1}dg)\gamma'_j,
\end{aligned}
\\ \textrm{tr}(g^{-1}dgg^{-1}\wedge dg)=0.
\end{gathered}
\end{equation}
The term $dA$ is slightly more complicated~:
\begin{equation}
\begin{aligned}
(dA)^i_j = d(A^i_j) =& -\textrm{tr}(g^{-1}dgg^{-1}dg(e_j))\wedge \omega^i + \textrm{tr}(g^{-1} d(dg(e_j)))\wedge \omega^i \\&+ \textrm{tr}(g^{-1}dg(e_j))d\omega^i.
\end{aligned}
\end{equation}
Using the structure equation~\eqref{eq:structure2} the last term is seen to be:
\[\textrm{tr}(g^{-1}dg(e_j)) d\omega^i=-\textrm{tr}(g^{-1}dg(e_j))(\Pi^i_k\wedge \omega ^k).\]
Since, 
\begin{equation}
\begin{aligned}
\Pi^i_k\wedge\omega^k(\cdot,e_i)&=\Pi^i_k(e_m)\omega^m\wedge\omega^k(\cdot,e_i)
\\&=\Pi^i_k(e_m)(\omega^m\delta^k_i - \delta^m_i \omega^k)
\\&=-\Pi^i_k(e_i)\omega^k,
\end{aligned}
\end{equation}
we conclude that~: 
\begin{equation}
\label{eq:ann_step6}
\textrm{tr}(g^{-1}dg(e_j))d\omega^i(\cdot,e_i) = \textrm{tr}(g^{-1}dg(e_j))\sum_m\sum_k\Pi^k_m(e_k)\omega^m.
\end{equation}
The remaining terms evaluate to the following expressions~:
\begin{equation}
\label{eq:ann_step7}
\begin{gathered}
 \textrm{tr}(g^{-1} d(dg(e_j)))\wedge \omega^i(\cdot,e_i)=(n-1)\textrm{tr}(g^{-1}d(dg(e_j))), \\
 -\textrm{tr}(g^{-1}dgg^{-1}dg(e_j))\wedge \omega^i=-(n-1)\textrm{tr}(g^{-1}dgg^{-1}dg(e_j)),\\
  -\textrm{tr}(g^{-1}dgg^{-1}dg(e_j))\wedge \omega^i + \textrm{tr}(g^{-1} d(dg(e_j)))\wedge \omega^i(\cdot,e_i)=(n-1)d\gamma'_j.
\end{gathered}
\end{equation}
Putting together equations~\eqref{eq:ann_step4},\eqref{eq:ann_step5},\eqref{eq:ann_step6} and \eqref{eq:ann_step7}, it follows that:
\begin{equation}\begin{split}\tilde{\Omega}^i_j(\cdot,\tilde{e}_i)=\Omega^i_k(\cdot,e_i)g^k_j -\frac{n-1}{n+1}d\gamma'_kg^k_j +\frac{n-1}{n+1}(\gamma'\Pi_U)_kg^k_j\\-\frac{n-1}{(n+1)^2}\textrm{tr}(g^{-1})\gamma'_k g^k_j,\end{split}\end{equation}
which is nothing more than $(n-1)$ times Equation~\eqref{eq_alpha_transfo}.

==> annexe/weyl_curvature.tex <==
% !TEX root = ../smf_proj.tex
\chapter{Proofs that are not essential to the main text}
\section{Calculating $\nabla_{a}W_{cd\phantom{a}f}^{\phantom{cd}a}$}
The computation is based on the second Bianchi identity :
\[\nabla_{[a}R_{bc]\phantom{d}e}^{\phantom{bc]}d}=0.\]
In this case of interest this leads to :
\[\begin{aligned} 0 &= \nabla_a R_{cd\phantom{a}f}^{\phantom{cd}a} + \nabla_c R_{da\phantom{a}f}^{\phantom{cd}a} + \nabla_d R_{ac\phantom{a}f}^{\phantom{cd}a},\\&=\nabla_a R_{cd\phantom{a}f}^{\phantom{cd}a} - \nabla_c R_{df} +\nabla_d R_{cf},  \\&= \nabla_a W_{cd\phantom{a}f}^{\phantom{cd}a} +2\nabla_a \delta^a_{[c}P_{d]f}   + 3\nabla_{[c} \beta_{df]} -(n-1)Y_{cdf}, \\&= \nabla_a W_{cd\phantom{a}f}^{\phantom{cd}a} +3\nabla_{[c}\beta_ {df]} -(n-2)Y_{cdf}.\end{aligned}\]
Hence : 
\begin{equation} 
\label{eq:derivative_weyl}
 \nabla_a W_{cd\phantom{a}f}^{\phantom{cd}a} = (n-2)Y_{cdf} -3\nabla_{[c}\beta_ {df]}.
\end{equation}

\section{Proof of Lemma~\ref{lemme:tractorformcouple}}
\label{app:preuve_lemme_tractorformcouple}
Let us prove the transformation law~\eqref{eq:tractor_form_transform} for the components of a $k$-cotractor form when we change connection according to $\hat{\nabla}=\nabla +\Upsilon$. This can be done by induction. The case $k=1$ is well known, but we prove it here for completeness. Consider: 
\[F_{A}\overset{\nabla}=\begin{pmatrix} \sigma \\ \mu_a \end{pmatrix} \overset{\hat{\nabla}}=\begin{pmatrix} \hat{\sigma} \\ \hat{\mu}_a \end{pmatrix}\] then for any tractor $T^A\overset{\nabla}=\rho Y_A + \nu^bW^A_b\overset{\hat{\nabla}}= \hat{\rho} Y_A + \hat{\nu}^bW_A^b$:
\[F_AT^A=\rho\sigma +\mu_b\nu^b=\hat{\rho}\hat{\sigma}+\hat{\mu}_b\hat{\nu}^b.\]
Using Equation~\eqref{eq:tractor_transfo}, it follows that: 
\[\rho\sigma + \mu_b\nu^b = (\rho-\Upsilon_b\nu^b)\hat{\sigma}+\hat{\mu}_b\nu^b.\]
Hence: \[\rho(\sigma-\hat{\sigma}) +\nu^b(\mu_b+\Upsilon_b\hat{\sigma}-\hat{\mu}_b)=0,\]
since this holds for arbitrary $\rho, \nu^b$ we conclude that:
\[\left\{ \begin{array}{l} \hat{\sigma} =\sigma, \\ \hat{\mu}_b=\mu_b+\Upsilon_b \sigma.\end{array}\right.\]
Assume now that~\eqref{eq:tractor_form_transform} is true for $k$-forms, we prove that it then holds for $k+1$ forms.
Let $F_{A_1\dots A_{k+1}}\overset{\nabla}=(k+1)\mu_{a_2\dots a_{k+1}}Y_{[A_1}Z^{a_2}_{A_2}\cdots Z^{a_{k+1}}_{A_{k+1}]}+\xi_{a_1\dots a_{k+1}}Z^{a_1}_{A_1}\cdots Z^{a_{k+1}}_{A_{k+1}}$. As in the case $k=1$, let $T^A\overset{\nabla}=\rho X^A + \nu^bW^A_b$ be an arbitrary tractor, we calculate the contraction:
\[\begin{aligned}F_{A_1\dots A_{k+1}}T^{A_{k+1}}&= ((-1)^{k}\rho\mu_{a_1\dots a_{k}}+\xi_{a_1\dots a_kb}\nu^{b})Z_{A_1}^{a_1}\dots Z_{A_{k}}^{a_{k}}\\&\hspace{2.3cm} +(k+1)\mu_{a_2\dots a_{k+1}}Y_{[A_1}Z^{a_2}_{A_2}\cdots Z^{a_{k+1}}_{A_{k+1}]}\nu^bW_b^{A_{k+1}}.\end{aligned}\]
\noindent The final term requires special attention:
\[\begin{aligned}(k+1)\mu_{a_2\dots a_{k+1}}Y_{[A_1}Z^{a_2}_{A_2}\cdots Z^{a_{k+1}}_{A_{k+1}]}\nu^bW_b^{A_{k+1}}=\hspace{2in}\\\frac{1}{k!}\sum_{\sigma\in\mathfrak{S}_{k+1}}\!\!\!\!\varepsilon(\sigma)\mu_{a_2\dots a_{k+1}} Y_{A_\sigma(1)}Z^{a_2}_{A_{\sigma(2)}}\cdots Z^{a_{k+1}}_{A_{\sigma(k+1)}}W^{A_{k+1}}_b\nu^b.\end{aligned}\]
If $\sigma(1)=k+1$, then the summand is zero, hence:
\[\begin{aligned}\sum_{\sigma \in \mathfrak{S}_k}\varepsilon(\sigma)\mu_{a_2\dots a_{k+1}} Y_{A_{\sigma(1)}}Z^{a_2}_{A_{\sigma(2)}}\cdots Z^{a_{k+1}}_{A_{\sigma(k+1)}}W^{A_{k+1}}_b\nu^b= \hspace{1.4in}\\\ \sum_{i=1}^{k} \sum_{\underset{\sigma(1)=i}{\sigma \in \mathfrak{S}_{k+1}}}\varepsilon(\sigma)\mu_{a_2\dots a_{k+1}} Y_{A_i}Z^{a_2}_{A_{\sigma(2)}}\cdots Z^{a_{k+1}}_{A_{\sigma(k+1)}}W^{A_{k+1}}_b\nu^b.\end{aligned}\]
Reorganising the terms in the product, we have that:
\[\begin{aligned} &\mu_{a_2\dots a_{k+1}} Y_{A_i}Z^{a_2}_{A_{\sigma(2)}}\cdots Z^{a_{k+1}}_{A_{\sigma(k+1)}}W^{A_{k+1}}_b\nu^b\hspace{2in}\\ &\hspace{.5in}=\mu_{a_2\dots a_{k+1}} Y_{A_i}Z^{a_{\sigma^{-1}(1)}}_{A_1}\cdots Z^{a_{\sigma^{-1}(i-1)}}_{A_{i-1}}Z^{a_{\sigma^{-1}(i+1)}}_{A_{i+1}} \cdots Z^{a_{\sigma^{-1}(k)}}_{A_{k+1}}W^{A_{k+1}}_b\nu^b, \\ &\hspace{.5in}= \mu_{a_{\sigma(2)}\dots {a_{\sigma(k+1)}}}\nu^{a_{k+1}}Y_{A_i}Z^{a_1}_{A_1}\dots Z^{a_{i-1}}_{A_{i-1}}Z^{a_{i+1}}_{A_{i+1}} \dots Z^{a_k}_{A_k}, \\&\hspace{.3in}= (-1)^{i-1}\varepsilon(\sigma)\mu_{a_1a_2\dots a_{i-1}a_{i+1}\dots a_{k+1}}\nu^{a_{k+1}}Y_{A_i}Z^{a_2}_{A_2}\dots Z^{a_{i-1}}_{A_{i-1}}Z^{a_{i+1}}_{A_{i+1}} \dots Z^{a_k}_{A_k}.\end{aligned}\]
The final equation comes from the following observation. If we relabel: \[\mu_{a_{\sigma(2)}\dots a_{\sigma(k+1)}}= \mu_{\bar{a}_1\dots \bar{a}_k};$$ then for any $s\in \mathfrak{S}_k$, $$\mu_{\bar{a}_{s(1)}\bar{a}_{s(2)}\dots \bar{a}_{s(k)}}=\mu_{a_{\sigma(s(1)+1)}\dots a_{\sigma(s(k)+1)}}.\]
Since $\sigma( \{2,\dots k\}) =\llbracket 1, k+1 \rrbracket \setminus\{ i\}$, we can reorder the indices such that we have $\mu_{a_1\dots a_{i-1}a_{i+1}\dots a_{k+1}}$ if we choose $s$ such that :
\[s(j) = \begin{cases}\sigma^{-1}(j)-1 & \textrm{if $1\leq j < i$}, \\ \sigma^{-1}(j+1) -1 & \textrm{if $i\leq j \leq k$}. \end{cases}\]
The signature of this permutation can be determined\footnote{in a rather tedious way} to be $(-1)^{i-1}\varepsilon(\sigma)$. One can observe that in the quotient group $\mathbb{R}^*/\mathbb{R}^*_+$:
\[\begin{aligned} \varepsilon(s) &=\prod_{1\leq m<l\leq k}\!\!\!\!s(l)-s(m),\\&=\prod_{1\leq m < l < i}\!\!\!\!\sigma^{-1}(l)-\sigma^{-1}(m)\!\!\!\!\prod_{1\leq m <i \leq l \leq k}\!\!\!\!\sigma^{-1}(l+1)-\sigma^{-1}(m)\\&\hspace{2.3in}\times\prod_{i\leq m<l \leq k}\!\!\!\!\sigma^{-1}(l+1)-\sigma^{-1}(m+1),\\&=\prod_{1\leq m < l < i}\!\!\!\!\sigma^{-1}(l)-\sigma^{-1}(m)\!\!\!\!\prod_{1\leq m <i < l \leq k+1}\!\!\!\!\sigma^{-1}(l)-\sigma^{-1}(m)\\&\hspace{2.3in}\times\prod_{i+1\leq m<l \leq k+1} \sigma^{-1}(l)-\sigma^{-1}(m). \end{aligned}\]
%
This differs from $\varepsilon(\sigma^{-1})$ by the sign of : \[ \prod_{1\leq m < i} 1-\sigma^{-1}(m) \equiv (-1)^{i-1} \textrm{mod } \mathbb{R}_+^*.\]
%
Overall, we find that :
\[\begin{split}F_{A_1\dots A_{k+1}}T^{A_{1}}= ((-1)^{k}\rho\mu_{a_1\dots a_{k}}+\nu^b\xi_{ba_1\dots a_{k}})Z_{A_1}^{a_1}\dots Z_{A_{k}}^{a_{k}}\hspace{.5in} \\+k\mu_{a_2a_3\dots a_ka_{k+1}}\nu^{a_{k+1}}Y_{[A_1}Z^{a_2}_{A_2}\cdots Z^{a_{k}}_{A_{k}]}.\end{split}\]
This is a $k$-cotractor, therefore, according to the induction hypothesis we must have:
\[\left\{ \begin{array}{l} \mu_{a_2\dots a_{k}b}\nu^{b}=\hat{\mu}_{a_2\dots a_k b}\hat{\nu}^{b},\\
(-1)^k\hat{\rho}\hat{\mu}_{\substack{\\a_1\dots a_{k}}}\!\!\!+\hat{\nu}^b\hat{\xi}_{a_1\dots a_{k}b}\!=\!(-1)^k\rho\mu_{\substack{\\a_1\dots a_{k}}}\!\!\!+\xi_{a_1\dots a_{k}b}\nu^b \!+\! k\Upsilon_{[a_1}\mu_{a_2\dots a_k]b}\nu^{b}. \end{array}\right.\]
Plugging the first equation into the second and using Equation~\eqref{eq:tractor_transfo}, we have 
\[\hat{\xi}_{a_1\dots a_{k}b}\nu^b= \nu^b\left(\xi_{a_2\dots a_{k}b} + \underbrace{k\Upsilon_{[a_1}\mu_{a_2\dots a_{k}]b} + (-1)^k\Upsilon_b\mu_{a_1\dots a_{k}}}_{k\Upsilon_{[a_1}\mu_{a_2\dots a_kb]}}\right).\]
The tractor $T^A$ being arbitrary, it follows that :
\[\left\{\begin{array}{l} \mu=\hat{\mu}, \\ \hat{\xi} = \xi + \Upsilon \wedge \mu, \end{array} \right. \]
and the result follows by induction.
\section{Hodge star of wedge product}
\begin{prop}
\label{prop:hodgestarwedge}
Let $\xi$ and $\Upsilon$ be respectively a $k$-form and a $1$-form on a pseudo-Riemannian manifold $(M,g)$, then :
\begin{equation} \label{eq:hodgestarwedge} \star(\Upsilon \wedge \xi) =(-1)^k\Upsilon^\sharp\lrcorner(\star \xi) \end{equation}
\end{prop}
\begin{proof}
The reason is essentially the fact that contraction and wedge product are adjoint operators. Precisely, if $\xi$ is $k$-form and $\alpha$ an arbitrary $(k+1)$-form then:
\begin{equation} \label{eq:wedgecontractionduality} g(\Upsilon\wedge \xi, \alpha)=g(\xi,\Upsilon^\sharp\lrcorner \alpha).\end{equation}
Postponing for now the proof of~\eqref{eq:wedgecontractionduality}, we prove Equation~\eqref{eq:hodgestarwedge}.
For any $k+1$-form $\alpha$:
\[\begin{aligned}\alpha \wedge \star(\Upsilon \wedge \xi) &= g(\alpha,\Upsilon\wedge\xi)\omega_g\\&=g(\Upsilon^\sharp\lrcorner\alpha,\xi)\omega_g\\&=(\Upsilon^\sharp \lrcorner \alpha) \wedge \star \xi. \end{aligned}\]
%
Since, $\Upsilon^\sharp \lrcorner \underbrace{(\alpha \wedge \star \xi)}_{=0}=(\Upsilon^\sharp \lrcorner \alpha)\wedge \star \xi - (-1)^{k}\alpha \wedge (\Upsilon^\sharp\lrcorner \star \xi)$
it follows that for any $\alpha$:
\[\alpha\wedge \left( (-1)^k \Upsilon^\sharp \lrcorner \star \xi \right) = g(\alpha, \star(\Upsilon \wedge \xi))\omega_g.\]
This property uniquely defines the Hodge star, therefore :
\[\star(\Upsilon \wedge \xi) =(-1)^k\Upsilon^\sharp\lrcorner \star \xi.\]
%
We prove now~\eqref{eq:wedgecontractionduality}, for instance, using the abstract index notation:
\[\begin{aligned} g(\Upsilon&\wedge \xi, \alpha)=\frac{1}{(k+1)!}g^{a_1b_1}\cdots g^{a_{k+1}b_{k+1}}(k+1)\Upsilon_{[a_1}\xi_{a_2\dots a_{k+1}]}\alpha_{b_1\dots b_{k+1}},\\ &=\frac{1}{k!(k+1)!}\sum_{\sigma \in \mathfrak{S}_{k+1}}\varepsilon(\sigma)g^{a_1b_1}\cdots g^{a_{k+1}b_{k+1}}\Upsilon_{a_{\sigma(1)}}\xi_{a_{\sigma(2)}\dots a_{\sigma(k+1)}}\alpha_{b_1\dots b_{k+1}},\\&=\frac{1}{k!(k+1)!}\sum_{\sigma \in \mathfrak{S}_{k+1}}\varepsilon(\sigma)g^{a_1b_{\sigma(1)}}\cdots g^{a_{k+1}b_{\sigma(k+1)}}\Upsilon_{a_{1}}\xi_{a_2\dots a_{k+1}}\alpha_{b_1\dots b_{k+1}},\\&=\frac{1}{k!(k+1)!}\sum_{\sigma \in \mathfrak{S}_{k+1}}\varepsilon(\sigma)g^{a_1b_1}\cdots g^{a_{k+1}b_{k+1}}\Upsilon_{a_{1}}\xi_{a_2\dots a_{k+1}}\alpha_{b_{\sigma^{-1}(1)}\dots b_{\sigma^{-1}(k+1)}},\\&= \frac{1}{k!(k+1)!}\sum_{\sigma \in \mathfrak{S}_{k+1}}g^{a_1b_1}\cdots g^{a_{k+1}b_{k+1}}\Upsilon_{a_{1}}\xi_{a_2\dots a_{k+1}}\alpha_{b_{1}\dots b_{k+1}},\\&=\frac{1}{k!}g^{a_2b_2}\cdots g^{a_{k+1}b_{k+1}}\xi_{a_2\dots a_{k+1}}g^{a_1b_1}\Upsilon_{a_{1}}\alpha_{b_{1}\dots b_{k+1}},\\&=g(\xi,\Upsilon^\sharp\lrcorner \alpha).\end{aligned}\]
\end{proof}

%\section{More on the Projective Cotton Tensor}

